Chaos of Learning Beyond Zero-sum and Coordination via Game Decompositions

Machine learning processes, e.g. ''learning in games'', can be viewed as non-linear dynamical systems. In general, such systems exhibit a wide spectrum of behaviors, ranging from stability/recurrence to the undesirable phenomena of chaos (or ''butterfly effect''). Chaos captures sensitivity of round-off errors and can severely affect predictability and reproducibility of ML systems, but AI/ML community's understanding of it remains rudimentary. It has a lot out there that await exploration. Recently, Cheung and Piliouras employed volume-expansion argument to show that Lyapunov chaos occurs in the cumulative payoff space, when some popular learning algorithms, including Multiplicative Weights Update (MWU), Follow-the-Regularized-Leader (FTRL) and Optimistic MWU (OMWU), are used in several subspaces of games, e.g. zero-sum, coordination or graphical constant-sum games. It is natural to ask: can these results generalize to much broader families of games? We take on a game decomposition approach and answer the question affirmatively. Among other results, we propose a notion of ''matrix domination'' and design a linear program, and use them to characterize bimatrix games where MWU is Lyapunov chaotic almost everywhere. Such family of games has positive Lebesgue measure in the bimatrix game space, indicating that chaos is a substantial issue of learning in games. For multi-player games, we present a local equivalence of volume change between general games and graphical games, which is used to perform volume and chaos analyses of MWU and OMWU in potential games.

==> material.tex <==
\begin{proposition}
$\dim(\Tz) = n+m-1$, $\dim(\Nz) = (n-1)(m-1)$, $\dim(\Tc) = n+m-1$, and $\dim(\Nc) = (n-1)(m-1)$.
\end{proposition}
\begin{proof}
	We prove the first two equalities only, as the other two can be derived analogously.
	Consider the linear map $(u_1,\cdots,u_n,v_1,\cdots,v_{m-1}) \ra (\bbT,-\bbT)\in \Tz$,
	such that $T_{jk} = u_j + v_k$ for any $j\in J$ and $k\in K\setminus \{m\}$, and $T_{jm} = u_j$ for any $j\in J$.
	It is direct to verify that this linear map is bijective, and the proposition follows by observing the domain of the linear map has dimension $n+m-1$.
	Then $\dim(\Nz) = \dim(\calZ) - \dim(\Tz) = (n-1)(m-1)$.
\end{proof}


==> projection_graphical.tex <==
\section{Projection onto Graphical Games}

\red{[I want to remove this section, as it is not very relevant to our paper's theme now. Agree?]}

The dimension of an $N$-player game can be exponentially high\footnote{For instance, if each player has $2$ strategies, the dimension is $2^N\cdot N$.},
so it is expected that learning in such games will be difficult to be analysed.
In contrast, the dual-volume behavior of low-dimensional graphical games\footnote{If each player has $2$ strategies, the dimension is at most $4N^2$.} can be analysed more easily.
\red{Say something about the observation in CP.}
The family of graphical games forms a vector subspace of general games, so it is natural to consider the projection of a general game into this subspace, which is the theme of this section.
We denote the subspace by $\calH$. As before, we first identify an orthogonal basis of $\calH$.

To simplify the description of an orthogonal basis of $\calH$, we first make the following observations.
\begin{itemize}
\item Let $\calH_i$ denote the subspace that represents the payoffs to Player $i$.
Then to describe an orthogonal basis for $\calH$, it suffices to describe, for each Player $i$, an orthogonal basis of $\calH_i$, since obviously $\calH = \calH_1 \oplus \calH_2 \oplus \cdots \oplus \calH_N$.
\item Let $\calH_{i,j}$ denote the subspace that represents the payoffs to Player $i$ when she selects strategy $j\in S_i$.
Then to describe an orthogonal basis for $\calH_i$, it suffices to describe, for each strategy $j\in S_i$, an orthogonal basis of $\calH_{i,j}$, since obviously $\calH_i = \bigoplus_{j\in S_i} \calH_{i,j}$.
\end{itemize}
Thus, we focus on describing an orthogonal basis for $\calH_{i,j}$. Let $\barn := \sum_{\ell \in [N]} n_\ell$.

\begin{proposition}
Suppose there are $N$ players, and Player $i$ has $n_i$ strategies. Then $\dim(\calH_{i,j}) = \barn - n_i - (N-2)$,
and thus $\dim(\calH) = 2 \sum_{1\le i < \ell \le N} n_i n_\ell - (N-2)\barn$.
\end{proposition}
\begin{proof}
For each Player $\ell$, denote its strategy set by $S_\ell$.
Recall that in $\calH_{i,j}$, we only focus on the payoffs to Player $i$ when she picks strategy $j\in S_i$.

Consider the linear mapping $\calL$, in which each point in the domain is $\{a^{\ell}_{k}\}$, where $\ell\neq i$ denotes a player, and $k\in S_\ell$,
and the range of $\calL$ is $\calH_{i,j}$, where we identify $a^{\ell}_{k}$ as the payoff to Player $i$ in the edge-game formed by Players $i,\ell$ when Player $\ell$ picks strategy $k$.
Clearly, $\calL$ is surjective.
%and the range is a $N$-player game matrix.
%$a^{i,\ell}_{j,k}$ denote the payoff to Player $i$ in the edge-game of the pair of Players $i,\ell$, when Player $i$ selects $j$ and Player $\ell$ selects $k$.
%Clearly, the mapping is linear,
Also, the dimension of the domain is $\barn - n_i$.
Thus, once we show that the dimension of $\ker(\calL)$ is $(N-2)$, we are done.

Let $\{a^{\ell}_{k}\}$ denote a point such that the resulting vector in $\calH_{i,j}$ is zero.
Suppose that each Player $\ell$ selects strategy $j_\ell$, we have
\[
\sum_{\ell\neq i} a^{\ell}_{j_\ell} = 0.
\]
Note that this inequality holds for \emph{any} choice of $j_\ell$ of all other players. Thus, by considering this equality when Player $\ell$ changes her strategy from $j_\ell$ to $j'_\ell$, we have
\[
a^{\ell}_{j_\ell}~\text{is the same for any}~j_\ell \in S_\ell,~\text{and thus we can simply denote it by}~a^{\ell}.
\]
Then it is easy to see that $\{a^{\ell}_{k}\}$ maps to the zero vector in $\calH_{i,j}$ if and only if $\sum_{\ell\neq i} a^{\ell} = 0$.
In other words, the kernel of $\calL$ if of dimension $(N-2)$, since it is one-to-one with the vector space with points in the form of $\{a^\ell\}_{\ell\in [N]\setminus\{i,r\}}$ for an arbitrary $r\neq i$
(it is one-to-one since $a^r = -\sum_{\ell\neq i,r} a^\ell$).

Since $\calH$ is the direct sum of $\calH_{i,j}$ for all $i\in [N]$ and $j\in S_i$, we have $\dim(\calH) = \sum_{i\in [N],j\in S_i} \dim(\calH_{i,j}) =
\sum_{i\in [N]} n_i (\barn - n_i - (N-2)) = 2 \sum_{1\le i < \ell \le N} n_i n_\ell - (N-2)\barn$.
\end{proof}

Now we are ready to describe an orthogonal basis for $\calH_{i,j}$.
By symmetry, we may take $i=1$. Let $j_\ell$ denote a strategy of Player $\ell$. Then
when Player $1$ selects strategy $j$ and for every other Player $\ell$ she selects $j_\ell$, the payoff to Player $1$ in a graphical game is of the form
\[
p_{2,j_2} ~+~ p_{3,j_3} ~+~ \cdots ~+~ p_{N,j_N}.
\]
We will use $\hp := \{p_{\ell,j_\ell}\}$ for $\ell=2,\cdots,N$ and $j_\ell \in S_\ell$ to specify the graphical games in an orthogonal basis:
\begin{itemize}
\item The first $n_2$ graphical games are: for each $k\in S_2$, $p_{2,k}=1$, while all other entries in $\hp$ are zero.
\item For $\ell=3,\cdots,N$, each corresponds to $n_\ell-1$ graphical games, where the $t$-th game is: $p_{\ell,s} = -1$ for $1\le s\le t$, $p_{\ell,t+1} = t$, and all other entries in $\hp$ are zero.
\end{itemize}
It is easy to verify that these $\barn - n_1 - (N-2)$ graphical games are pairwise orthogonal. Then they can be used with~\eqref{eq:proj-on-subspace} to compute the projection of any general game on graphical game.



\red{As an illuminating example, project $N$-player Rock-Paper-Scissors game into graphical games.}

